Keyphrase Extraction from Scholarly Articles as Sequence Labeling using Contextualized Embeddings

In this paper, we formulate keyphrase extraction from scholarly articles as a sequence labeling task solved using a BiLSTM-CRF, where the words in the input text are represented using deep contextualized embeddings. We evaluate the proposed architecture using both contextualized and fixed word embedding models on three different benchmark datasets (Inspec, SemEval 2010, SemEval 2017) and compare with existing popular unsupervised and supervised techniques. Our results quantify the benefits of (a) using contextualized embeddings (e.g. BERT) over fixed word embeddings (e.g. Glove); (b) using a BiLSTM-CRF architecture with contextualized word embeddings over fine-tuning the contextualized word embedding model directly, and (c) using genre-specific contextualized embeddings (SciBERT). Through error analysis, we also provide some insights into why particular models work better than others. Lastly, we present a case study where we analyze different self-attention layers of the two best models (BERT and SciBERT) to better understand the predictions made by each for the task of keyphrase extraction.

==> dataset.tex <==
\section{Dataset}
KDD, WWW, Inspec, SemEval-2010, SemEval-2017, Kp20k
https://github.com/boudinfl/ake-datasets


==> problem_statement.tex <==
\section{Problem Statement}


==> related_work.tex <==
\section{Related Work}
The task of keyphrase extraction, previously, has been performed by using various supervised and unsupervised models \cite{hasan2014automatic}. For the supervised models, after the initial candidate phrase selection based on POS tags or n-grams. The candidate phrases are then input to a machine learning model which classifies it as a keyword or non-keyword on the basis of their features like : position of occurrence, frequency of occurrence, presence in the title of document etc \cite{Frank:1999:DKE:646307.687591} \cite{hulth2003improved} \cite{10.1007/978-3-540-77094-7_41} \cite{Caragea2016}. 

In the unsupervised scenario, the keyphrase extraction is carried out either on basis of graph-based ranking, topic-based clustering or aggregation of scores of individual words of a keyphrase on basis of measures like tf-idf or other statistical and linguistic measures \cite{Zhang2007comparative} \cite{Barker2000UsingNP}. In graph-based methods candidate keyphrases are treated as nodes which are ranked on basis of \textit{importance} which is determined by it's \textit{relatedness}(semantic or co-occurrent) to other candidate keyphrases eg: TextRank\cite{mihalcea2004textrank} SingleRank \cite{wan2008single} CollabRank \cite{wan-xiao-2008-collabrank}.In topic-based clustering candidates are grouped into topics and then keyphrases are selected equally \cite{Liu2009Exemplar} or unequally \cite{Grineva:2009:EKT:1526709.1526798} \cite{Liu:2010:AKE:1870658.1870694} from each topic.

Along with the features extracted from text, sometimes, external features are also incorporated to facilitate keyword extraction. In supervised setting, documents citation network or webpage's hyperlink network have been used as external features \cite{caragea2014citation} \cite{Kelleher2005hypertext} \cite{Bulgarov2015comparison}. Whereas, in unsupervised setting, language models which were trained on web \cite{Tomokiyo2003language} have been used and sometimes relation between words has been assigned on basis of information from Wordnet \cite{martinez2015semgraph}.

Various deep learning models have also been employed for the task of keyphrase extraction. In \cite{Rui2017generation} have introduced a RNN based generative model. It employs a copying mechanism with RNN model, with the help of which, they can not only extract explicit keywords( keywords that are present in the text) but also predict/generate implicit keywords. \cite{zhang-etal-2016-keyphrase} have also used a RNN based network to perform keyword extraction on a dataset collated from twitter. Using their model, they have tried to address the problem of keyphrase extraction in case limited length of data.

Recently, sequence labeling models have been used by various researchers for the task of keyphrase extraction. \cite{gollapalli2016keyphrase} have used Conditional random fields along with features like tf-idf, POS tags and position of occurrence to identify keywords from the text. In the paper, they have tokenized the full text and then assigned the label Keyphrase(\textbf{KP}) and non-keyphrase(\textbf{Non-KP}) to keyphrases and non-keyprases respectively. While their model successfully captures dependencies in output label, in didn't capture the input sequence dependencies. \cite{berend-2017-szte} have also used CRF's for the sequence labelling but instead of using basic features they have used features like sparse coding of dense word embeddings \cite{berend-2017-sparse} brown clustering \cite{Brown1992clustering} etc. In \cite{Alzaidy:2019:BSL:3308558.3313642} along with final CRF layer, authors have also used a Bi-LSTM layer between the input and the CRF layer, with the help of this extra layer they are able to capture input sequence dependencies as well.




